Information Criteria for quantifying loss of reversibility in parallelized KMC

Parallel Kinetic Monte Carlo (KMC) is a potent tool to simulate stochastic particle systems efficiently. However, despite literature on quantifying domain decomposition errors of the particle system for this class of algorithms in the short and in the long time regime, no study yet explores and quantifies the loss of time-reversibility in Parallel KMC. Inspired by concepts from non-equilibrium statistical mechanics, we propose the entropy production per unit time, or entropy production rate, given in terms of an observable and a corresponding estimator, as a metric that quantifies the loss of reversibility. Typically, this is a quantity that cannot be computed explicitly for Parallel KMC, which is why we develop a posteriori estimators that have good scaling properties with respect to the size of the system. Through these estimators, we can connect the different parameters of the scheme, such as the communication time step of the parallelization, the choice of the domain decomposition, and the computational schedule, with its performance in controlling the loss of reversibility. From this point of view, the entropy production rate can be seen both as an information criterion to compare the reversibility of different parallel schemes and as a tool to diagnose reversibility issues with a particular scheme. As a demonstration, we use Sandia Lab's SPPARKS software to compare different parallelization schemes and different domain (lattice) decompositions.

==> sections/formalCalc.tex <==
% Formal calculation of the RER and EPR without assumptions on schemes and 
% details.
\subsection{Asymptotic Expansions} 
 Let us consider $\Po(\si,\si')=e^{\Dt
 L}\de_{\si'}(\si)$, where $L$ is the infinitesimal generator of the 
discrete Markov chain. By splitting the generator $L$ into $L_1+L_2$,
we can construct approximations to $\Po$. In this section, we are going to carry
out the calculations with respect to the Lie approximation,
$\Pb(\si,\si')=e^{\Dt L_1}e^{\Dt L_2}\de_{\si'}(\si)$. However, the arguments
apply to other splittings as well. 

By using the power series representations of $e^{\Dt L_1}$ and
$e^{\Dt L_2}$, we can calculate their product as a Cauchy product series to get

\begin{align}
  \label{eq:approx-pow-series}
 \Pb(\si,\si')=\des+\Dt L\des + \frac{\Dt^2}{2}(L_1^2+L_2^2+2L_1L_2)+o(\Dt^3).
\end{align}

Therefore, we have 

\begin{align}
  \label{eq:error-pow-series}
  \Po(\si,\si')-\Pb(\si,\si)=\frac{\Dt^2}{2}[L_1,L_2]\des+o(\Dt^3), 
\end{align}
This is the form of the error that we introduced in
Lemma~\ref{lem:p_and_C}, with the commutator $C=[L_1,L_2]$ and $p=2$.

The operating assumption in this section was that all generators are bounded.
This allowed us to represent the transition densities with power series and,
subsequently, to calculate the form of the commutators and of other quantities
of interest. However, the present work could also be extended to the case of
unbounded operators~\cite{hansen,Janhke}, where alternative representations for the semigroups could
be used for the error analysis. We are not handling
such cases here, as the Markov generators of stochastic particle systems are
bounded~\cite{Arampatzis:2014}. 



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% End: 
